Quantified Facial Expressiveness for Affective Behavior Analytics

The quantified measurement of facial expressiveness is crucial to analyze human affective behavior at scale. Unfortunately, methods for expressiveness quantification at the video frame-level are largely unexplored, unlike the study of discrete expression. In this work, we propose an algorithm that quantifies facial expressiveness using a bounded, continuous expressiveness score using multimodal facial features, such as action units (AUs), landmarks, head pose, and gaze. The proposed algorithm more heavily weights AUs with high intensities and large temporal changes. The proposed algorithm can compute the expressiveness in terms of discrete expression, and can be used to perform tasks including facial behavior tracking and subjectivity quantification in context. Our results on benchmark datasets show the proposed algorithm is effective in terms of capturing temporal changes and expressiveness, measuring subjective differences in context, and extracting useful insight.

==> app_MM.tex <==
\section{Multimedia Application}

==> conclusion.tex <==
% \vspace{-2mm}

% \section{Conclusion}

% In this work, we proposed an algorithm to quantify facial expressiveness using multimodal facial features that captures spatial (static) and temporal expressiveness. The proposed algorithm provides a bounded continuous expressiveness score, which is essential for the relative measurement of expressiveness. The QFE algorithm was evaluated on multiple benchmark affect datasets and demonstrated promising results on performing downstream affective computing tasks including subjectivity quantification. We also demonstrated how the proposed algorithm can be used to analyze, interpret, summarize to tell story using the proposed method leveraging facial expressiveness and multimedia contents (e.g. stimulus video, temperature from heat sensor). In our future work, we intend to study QFE in the context of non-face modalities such as human physiology and speech to investigate the relationship between facial expressiveness, physiology, and speech in context to test hypotheses regarding affective science and to study affective computing in multimedia. We also intend to incorporate demographic information in our analysis to create better summarization of data. We also intended to evaluate the proposed method in the context of creative tasks such ch singing, dancing, (math) problem solving. 




==> dataset.tex <==
\section{Datasets}

\textbf{DISFA dataset}. DISFA dataset \cite{mavadati2013disfa} is a publicly available spontaneous facial expression dataset which contains $27$ subjects (12 females, and 15 males) aged in between $[18, 50]$ and ethnically $3$ Asian, $21$ Caucasian, $1$ Black, and $2$ Hispanic  subjects. The dataset contains frontal face images and action unit (AU) \cite{ekman1976measuring} annotations at frame level, by expert annotators. The dataset contains $27$ videos comprising $130,000$ images. A video comprising of $9$ segments with different types of content was used as the stimuli to elicit the expression. The stimuli video and corresponding frontal face videos of the subjects are each $242$ seconds long. \textit{We chose this dataset for our experimental design due to the correspondence of the stimuli video and subjects, which makes it useful to study subjective differences.}

\textbf{BioVid pain dataset}. BioVid pain dataset \cite{walter2013biovid} contains $90$ subjects performing pain and other expressions. The dataset is balanced in terms of gender. There are three age groups in the dataset in the age range of $ [18-35], [36-50], [51-65]$ years old. In this work, we used the raw data which is part C in the data portion and contains $87$ subjects. Continuous heat (temperature) was used as a stimulus to elicit pain expression, which was self-calibrated by the subjects. The length of each session is approximately $25$ minutes, and in total, in Part C, is comprised of approximately $3.26$ million images. Aside from the frontal face videos and temperature, the dataset contains pain labels in between $[0, 4]$, where $0$ means no pain, and $4$ means maximum pain. \textit{We chose this dataset for our experimental design due to the availability of temporal context (temperature), which is highly controlled in the data collection process.}



==> rebuttal.tex <==
\section*{Rebuttal}
We thank the reviewers for their insightful critiques, helping make the paper better, and their positive feedback.

\textbf{R1}. "Overall, it is \textbf{interesting work}. The issues I pointed out can be \textit{fixed in a few hours and verified by the AC/designated reviewer before final acceptance}."

\textbf{R2}. "The ablation study on frame rate and temporal modalities is good to see. The algorithm is run on several datasets and numerous statistics computed."

\textbf{R3}. Proposed QFE is clearly explained and is technically sound. The metric is shown to efficiently quantify expressiveness, and \textbf{in line with the theories of emotion}. Overall, the idea of quantifying subjective facial expressiveness is \textbf{interesting and practically useful in a variety of affective computing tasks}, including emotion annotation and detection..."% The proposed metric is relevant in this regard: it is technically sound and shown to correlate well with existing studies in facial expressiveness. For these reasons, I \textbf{recommend this paper for publication}, albeit with some revisions mentioned below.

\noindent \textbf{Critiques and how they are addressed}

\textbf{R1.1} "Some discussion about such important subtleties is needed..." \textcolor{blue}{ We updated our discussion (Sec. \ref{sec:relWorks} \& Sec. \ref{sec:disc}) to highlight the importance of valence, and arousal. In addition, the proposed approach can also be used to compute complex/mixed affective expressions using the subset of AUs that are associated to each affect/emotion category. For example, if happiness, and surprise co-occurred at the same time, we can compute expressiveness for both happiness, and surprise separately. For instance, in Section \ref{sec:GrangerTestRes}, we computed pain expressiveness using AUs that are associated with pain. } 

\textbf{R1.2} Presentations issues and $p=0$. \textcolor{blue}{We updated the presentation, and updated $p=0$ to $<0.001$.}

\textbf{R2.1} "Obviously expressivity is a subjective matter, but it can be approximated by interviewing numerous people to get an average score.., it's impossible to judge how good this method is." \textcolor{blue}{"The goal of this work is to perform affective data analytics. Also, example tasks we experimented with are relevant affective computing tasks. Please see updated and expanded Section \ref{sec:exp} for new details to help judge the quality of the proposed approach - we used human ratings / annotations following the suggestion.}%  We can do some manual validation on DISFA dataset. Comparisons with bioVid dataset for subjects mentioned in dataset that did not show target expressivity. Subjectivity analysis did tell us the usefulness of the method. We found statistically significant association among 25 subjects output 27 subjects. 25 subjects did showed expressiveness in response to the stimuli with variabilities in terms of level of expressiveness and delay (lapse)."}

\textbf{R2.2} "However, it's not clear until way into the paper "what" the authors are trying to do..."% What specific problem is trying to be solved?" "What specific problem is motivating this work? Explicitly stating this earlier will make reading and understanding much easier, especially for readers less familiar with this area." 
\textcolor{blue}{We are measuring how expressive a human face is in a video at the frame-level so that we can use this info to perform affective data analytics. The details of what this work is proposing is found in the Introduction, more specifically in the enumerated contributions of the work in the Introduction. }

\textbf{R2.3} "why is expressivity important and what is current SOTA?" "This in turn makes assessing the impact of the proposed approach very difficult (is it fundamentally new, or just a minor modification)?" \textcolor{blue}{It gives much richer set of information about expressions (Introduction), and SOTA is covered in Related works 'paragraph 2'. We do have description on method and experiments section. Expressivity is new (we as a community previously work on expression). First AI paper published on this topic was on late 2019. Our algorithm is new, not a minor modification.}

\textbf{R2.4} "Unclear how the claim starting in 161 follows because there's no prior discussion around annotation." \textcolor{blue}{"There is no work on expressivity at frame-level except the work from Uddin et al. \cite{uddin2020quantified}. Before we make this claim, we give details about limitations of current annotations in the Introduction and Related Works.}

\textbf{R2.5} "... measurements don't show that the method is useful in performing a downstream task better." \textcolor{blue}{Knowing difference between subjects, and knowing the alignment between context and facial expression are affective computing tasks. We would like to point out the strength listed by R3, in the proposed approach is \textit{"interesting and practically useful in a variety of affective computing tasks"}, which is the proposal of this work. We have added new evaluations in Section \ref{sec:exp} to help clarify this point.}

\textbf{R2.6}" The authors have shown that their algorithm correlates with various features..., there is no way to confirm whether this is correct or better than other approaches..." \textcolor{blue}{"To better evaluate this, we have conducted new experiments with human annotators on DISFA \& BioVid pain (see Sec. \ref{sec:qfe} for these new details). Also, in the subjectivity quantification results, most subjects were correlated with $p-value < 0.05$, which is an indication that most subjects showed expressions as our method shows.}

%We can use human to go over the annotation we got from our algorithm on DISFA dataset. We can actually from DISFA dataset. The data was collected using several stimuli videos, and rated by human annotator for each video frames. So, this dataset is solid in that regards. Also, if you look carefully

\textbf{R3.1} "Do the authors employ any robustness against such detection errors when computing QFE?".  \textcolor{blue}{We can use OpenFace or other tools to extract features. %The good thing about OpenFace is that it is accessible to everyone (open-sourced), and one stop-shopping for affective visual computing.
We can pre-process the extracted features before computing QFE. Details on this have been added to Section  \ref{sec:disc}.}

%For instance, in case of $\sigma$, the influence of outliers can be reduced using the fact that $0 <= AU_{intensities} <= 5$. To deal with the noises and outliers, we can leverage the confidence of the feature extraction models to deal with poorly extracted features. For instance, OpenFace outputs face detection probabilities, which can be used to pre-process data and to take action to reduce the adverse effects of the noise and anomaly. Also, anomaly detection techniques can be employed to detect anomaly.}

\textbf{R3.2}"...the paper needs discussion on the sensitivity of the QFE metric to errors in automated feature detection..." \textcolor{blue}{We performed experiments simulating noise and anomalies. Please see new details in Section \ref{sec:disc} and Figure \ref{fig:noise_simulation}.}

\textbf{R3.3} "the authors can consider testing their metric, especially for verifying Granger causality, in more challenging scenarios..." \textcolor{blue}{Granger causality requires the variables to be temporal \& continuous. Considering this, we evaluated DISFA by manually observing the facial expressiveness in parallel with the stimuli video, and annotated whether a given subject responded to a given video (context). New details on this have been added to Section \ref{sec:qfe} and Fig. \ref{fig:DISFA_subResponded_to_stimuli}.}

\textbf{R3.4}"Minor concerns and typo..:" \textcolor{blue}{$x_i$ is a vector of 17 elements; Headpose captures info that's in 3D LM. Also, length of 2D LM and length of HP is less than length of 3D LM; weights are problem specific. In approach 1 and 2, we manually select the weight, and in approach 3, we used a statistical model; We empirically found LM and HP are more influential than G, so we put more weight on LM and HP. In other tasks (e.g. driver's behavior modeling), G could be more influential; typos fixed.}


% Also, our contribution is not using the OpenFace, it's our algorithm and algorithm we proposed can work with OpenFace and other systems as well. Current version of the paper did not look into this issue.
\clearpage
